Training-free LLM Merging for Multi-task Learning

Large Language Models (LLMs) have demonstrated exceptional capabilities across diverse natural language processing (NLP) tasks. The release of open-source LLMs like LLaMA and Qwen has triggered the development of numerous fine-tuned models tailored for various tasks and languages. In this paper, we explore an important question: is it possible to combine these specialized models to create a unified model with multi-task capabilities. We introduces Hierarchical Iterative Merging (Hi-Merging), a training-free method for unifying different specialized LLMs into a single model. Specifically, Hi-Merging employs model-wise and layer-wise pruning and scaling, guided by contribution analysis, to mitigate parameter conflicts. Extensive experiments on multiple-choice and question-answering tasks in both Chinese and English validate Hi-Merging's ability for multi-task learning. The results demonstrate that Hi-Merging consistently outperforms existing merging techniques and surpasses the performance of models fine-tuned on combined datasets in most scenarios. Code is available at: https://github.com/Applied-Machine-Learning-Lab/Hi-Merging.

==> Miscellaneous.tex <==

% In our experiments, we compare \mname with a comprehensive set of baseline methods based on weighted averaging and delta vectors. Additionally, we consider an idealized baseline called the multilingual and multi-task model, where a single model is trained on combined datasets simultaneously.

% Basic weighted averaging techniques, like Model Soups~\cite{modelsoup}, aim to merge model weights by directly averaging LLMs without considering their pre-trained base model. On the other hand, Task Arithmetic~\cite{taskarithmetic} is the first approach that focuses on merging delta vectors (the parameter differences between the pre-trained and fine-tuned models) of the LLMs. Subsequent methods focus on reducing conflicts between delta vectors during merging. For example, TIES-Merging~\cite{ties} minimizes task interference by trimming small delta vector values and averaging the left ones a consensus sign. DARE~\cite{dare} reduces conflicts across tasks by randomly sparsifying delta vectors, while DELLA~\cite{della} assigns drop rates to delta vectors according to their absolute values to improve performance stability. Model Breadcrumbs~\cite{modelbread} prunes maxima and minima in delta vectors to retain critical task-specific features.




\begin{table*}[ht]
    \centering
    \caption{Performance comparison of model merging methods on the MCQA task in a multilingual setting.}
    \label{tab:multilingual-mcqa}
    \begin{subtable}{0.48\textwidth}
        \centering
        \caption{Qwen2-7B-Instruct}
        \resizebox{\textwidth}{!}{
        \begin{tabular}{@{}llccc@{}}
            \toprule
            \textbf{Types} & \textbf{Methods} & \textbf{L1 (MedQA)} & \textbf{L2 (CMExam)} & \textbf{Avg.} \\ \midrule
            \multirow{3}{*}{Pre-trained} 
                & Qwen2-7B-Instruct & 51.4062 & 74.6217 & 63.0140 \\
                & Yi-1.5-9B       & 46.8185 & 58.6499 & 52.7342 \\
                & Baichuan2-7B    & 6.4415  & 7.1439  & 6.7927  \\ \midrule
            \multirow{3}{*}{Fine-tuned} 
                & Model A (L1)    & 59.1406 & 83.7771 & 71.4589 \\
                & Model B (L2)    & 54.4531 & 88.6171 & 71.5351 \\
                & Multilingual    & 60.0781 & 88.2246 & 74.1514 \\ \midrule
            \multirow{9}{*}{Merged} 
                & Model Soups     & 59.6094 & 88.6926 & 74.1510 \\
                & Task Arithmetic & 59.5312 & 88.7681 & 74.1497 \\
                & TIES            & 59.0625 & \underline{\textbf{88.7832}} & 73.9229 \\
                & DARE            & 58.6719 & 88.6926 & 73.6823 \\
                & DARE + TIES     & 58.9063 & 88.6021 & 73.7542 \\
                & Model Breadcrumbs & 58.8281 & 88.6322 & 73.7302 \\
                & DELLA           & 58.9844 & 88.7681 & 73.8763 \\
                & DELLA + TIES    & 58.2812 & 88.7530 & 73.5171 \\
                & \mname (Ours)   & \underline{\textbf{61.0156}} & 88.6501 & \underline{\textbf{74.8329}} \\ 
            \bottomrule
        \end{tabular}
        }
    \end{subtable}
    \begin{subtable}{0.48\textwidth}
        \centering
        \caption{Llama-3-8B-Instruct}
        \resizebox{\textwidth}{!}{
        \begin{tabular}{@{}llccc@{}}
            \toprule
            \textbf{Types} & \textbf{Methods} & \textbf{L1 (MedQA)} & \textbf{L2 (CMExam)} & \textbf{Avg.} \\ \midrule
            \multirow{3}{*}{Pre-trained} 
                & Llama-3-8B-Instruct      & 57.9733 & 17.2821 & 37.6277 \\
                & GLM-4-9B        & 54.7656 & 69.5194 & 62.1425 \\
                & Gemma-2-9B      & 14.2583 & 2.7698  & 8.5141  \\ \midrule
            \multirow{3}{*}{Fine-tuned} 
                & Model A (L1)    & 60.4688 & 52.2706 & 56.3697 \\
                & Model B (L2)    & 60.3906 & 60.5525 & 61.0575 \\
                & Multilingual    & \textbf{62.8906} & 61.0356 & \textbf{61.9631} \\ \midrule
            \multirow{9}{*}{Merged} 
                & Model Soups     & 61.2500 & 61.0507 & 61.1504 \\
                & Task Arithmetic & 61.2500 & \underline{\textbf{61.8750}} & 61.5625 \\
                & TIES            & 61.7188 & 61.3225 & 61.5207 \\
                & DARE            & 61.5625 & 61.3678 & 61.4652 \\
                & DARE + TIES     & 60.9375 & 59.4656 & 60.2016 \\
                & Model Breadcrumbs & 61.0156 & 60.4318 & 60.7237 \\
                & DELLA           & 60.8594 & 60.7186 & 60.7890 \\
                & DELLA + TIES    & 61.9531 & 61.3527 & 61.6529 \\
                & \mname (Ours)   & \underline{62.2656} & 61.0757 & \underline{61.6707} \\ 
            \bottomrule
        \end{tabular}
        }
    \end{subtable}
    % \hspace*{-\leftmargin}
    \begin{tablenotes}[flushleft]
        \footnotesize
        \item \textit{Note:} The best result across all models marked in bold. The best result of the merging methods is underlined.
    \end{tablenotes}
\end{table*}


\begin{table*}[h]
    \centering
    \caption{Performance comparison of model merging methods on the QA task in a multilingual setting.}
    \label{tab:multilingual-qa}
    \begin{subtable}{\textwidth}
        \centering
        \caption{Qwen2-7B-Instruct}
        \resizebox{\textwidth}{!}{
        \begin{tabular}{@{}llccccccccc@{}}
            \toprule
            \multirow{2}{*}{\textbf{Types}} &
              \multirow{2}{*}{\textbf{Methods}} &
              \multicolumn{4}{c}{\textbf{L1 (HealthCareMagic)}} &
              \multicolumn{4}{c}{\textbf{L2 (cMedQA2)}} &
              \multirow{2}{*}{\textbf{Avg.}} \\ \cmidrule(lr){3-10}
                                        &                   & BLEU-4  & ROUGE-1 & ROUGE-2 & ROUGE-l & BLEU-4 & ROUGE-1 & ROUGE-2 & ROUGE-l &         \\ \midrule
            Pre-trained                 & Qwen2-7B-Instruct & 30.1209 & 26.3524 & 5.3280  & 15.7451 & 1.7090 & 14.1527 & 1.7822  & 9.0934  & 13.0355 \\ \midrule
            \multirow{3}{*}{Fine-tuned} & Model A (L1)      & 35.5717 & 30.2512 & 8.9044  & 20.3625 & 3.7609 & 19.1370 & 3.1364  & 15.1441 & 17.0335 \\
                                        & Model B (L2)      & 24.8587 & 24.9841 & 4.1492  & 15.1967 & 4.4159 & 21.2210 & 4.0680  & 17.4600 & 14.5442 \\
                                        & Multilingual      & 35.7637 & 29.9781 & 8.6687  & 20.1184 & 3.7660 & 20.9869 & 3.7784  & 16.8850 & 17.4932 \\ \midrule
            \multirow{9}{*}{Merged}     & Model Soups       & 33.2627 & 28.8258 & 7.5487  & 18.9459 & 4.6801 & {\ul \textbf{21.5564}} & 4.0502  & 17.5380 & 17.0510 \\
                                        & Task Arithmetic   & 33.0398 & 28.7169 & 7.5726  & 18.9600 & 4.7181 & 21.4108 & 4.0503  & 17.6772 & 17.0182 \\
                                        & TIES              & 33.6571 & 29.0496 & 7.7769  & 19.1503 & 4.3751 & 20.8551 & 3.7518  & 17.1978 & 16.9767 \\
                                        & DARE & 33.3031 & 28.9575 & 7.8222 & 19.1702 & {\ul \textbf{4.7578}} & 21.0865 & 3.8996 & 17.2488 & 17.0307 \\
                                        & DARE+TIES         & 26.8091 & 26.0330 & 5.2307  & 16.5201 & 4.2456 & 20.6276 & 3.7531  & 17.1445 & 15.0455 \\
                                        & Model Breadcrumbs & 34.3247 & 29.4403 & 8.1518  & 19.6443 & 4.4092 & 20.9365 & 3.8138  & 17.1378 & 17.2323 \\
                                        & DELLA             & 33.4207 & 28.9234 & 7.6728  & 18.9674 & 4.6827 & 21.1596 & 4.0709  & 17.4775 & 17.0469 \\
                                        & DELLA+TIES        & 27.2331 & 26.1723 & 5.4339  & 16.6009 & 4.7130 & 21.2275 & {\ul \textbf{4.2944}} & {\ul \textbf{17.7694}} & 15.4306 \\
                                        & \mname (Ours) & {\ul \textbf{35.9500}} & {\ul \textbf{29.9826}} & {\ul \textbf{8.8738}} & {\ul \textbf{20.3844}} & 4.7009 & 21.1752 & 3.9704 & 17.2361 & {\ul \textbf{17.7842}} \\ 
            \bottomrule
        \end{tabular}
        }
    \vspace{0.5\baselineskip}
    \end{subtable}
    % \hfill
    
    \begin{subtable}{\textwidth}
        \centering
        \caption{Llama-3-8B-Instruct}
        \resizebox{\textwidth}{!}{
        \begin{tabular}{@{}llccccccccc@{}}
            \toprule
            \multirow{2}{*}{\textbf{Types}} &
              \multirow{2}{*}{\textbf{Methods}} &
              \multicolumn{4}{c}{\textbf{L1 (HealthCareMagic)}} &
              \multicolumn{4}{c}{\textbf{L2 (cMedQA2)}} &
              \multirow{2}{*}{\textbf{Avg.}} \\ \cmidrule(lr){3-10}
                                            &                   & BLEU-4  & ROUGE-1 & ROUGE-2 & ROUGE-l & BLEU-4 & ROUGE-1 & ROUGE-2 & ROUGE-l &         \\ \midrule
            Pre-trained                     & Llama-3-8B-Instruct        & 16.3118 & 21.6011 & 3.1389  & 10.8666 & 0.0225 & 0.4710  & 0.0211  & 0.2343  & 8.7780  \\ \midrule
            \multirow{3}{*}{Fine-tuned}     & Model A (L1)      & 36.0325 & 30.4111 & 9.2743  & 20.7236 & 0.0185 & 0.1288  & 0.0025  & 0.0841  & 16.3381 \\
                                            & Model B (L2)      & 3.9950  & 7.7673  & 0.9267  & 4.6358  & 3.0638 & 20.4016 & 3.4178  & 16.3067 & 9.1899  \\
                                            & Multilingual      & 35.6154 & 30.5447 & 9.2156  & 20.4271 & 3.0250 & 20.3136 & 3.4964  & 16.0911 & 19.0912 \\ \midrule
            \multirow{9}{*}{Merged}         & Model Soups       & 32.1199 & 28.2278 & 6.3715  & 18.2456 & 3.3256 & 19.5499 & 2.8670  & 15.4688 & 15.7473 \\
                                            & Task Arithmetic   & 31.6679 & 27.7646 & 6.0354  & 18.0448 & 3.3805 & 19.6475 & 2.9507  & 15.4806 & 15.6153 \\
                                            & TIES              & 32.1494 & 28.0527 & 6.7440  & 18.2913 & 3.2238 & 19.5369 & 2.8854  & 15.2112 & 15.6818 \\
                                            & DARE              & 25.9679 & 25.6716 & 4.5173  & 16.3803 & 3.5337 & 20.8586 & 3.1736  & 16.6716 & 14.8506 \\
                                            & DARE+TIES         & 26.6707 & 25.9106 & 5.2031  & 16.5525 & 3.2236 & 19.8564 & 2.9963  & 15.5967 & 15.0016 \\
                                            & Model Breadcrumbs & 26.9844 & 26.1004 & 4.7037  & 16.3247 & 3.3307 & 20.7442 & 3.3069  & 16.2874 & 15.2977 \\
                                            & DELLA             & 25.6313 & 25.6792 & 4.5522  & 16.1313 & 3.6612 & 20.9176 & 3.3286  & 16.7355 & 15.1501 \\
                                            & DELLA+TIES        & 27.1246 & 26.0186 & 5.3163  & 16.6170 & 3.3433 & 19.9122 & 3.0848  & 15.9942 & 15.4260 \\
                                            & \mname (Ours)     &         &         &         &         &        &         &         &         &         \\ 
            \bottomrule
        \end{tabular}
        }
    \end{subtable}
    % \hspace*{-\leftmargin}
    \begin{tablenotes}[flushleft]
        \footnotesize
        \item \textit{Note:} The best result across all models marked in bold. The best result of the merging methods are are underlined.
    \end{tablenotes}
\end{table*}
